GraphPatcher: Mitigating Degree Bias for Graph Neural Networks via Test-time Augmentation

Recent studies have shown that graph neural networks (GNNs) exhibit strong biases towards the node degree: they usually perform satisfactorily on high-degree nodes with rich neighbor information but struggle with low-degree nodes. Existing works tackle this problem by deriving either designated GNN architectures or training strategies specifically for low-degree nodes. Though effective, these approaches unintentionally create an artificial out-of-distribution scenario, where models mainly or even only observe low-degree nodes during the training, leading to a downgraded performance for high-degree nodes that GNNs originally perform well at. In light of this, we propose a test-time augmentation framework, namely GraphPatcher, to enhance test-time generalization of any GNNs on low-degree nodes. Specifically, GraphPatcher iteratively generates virtual nodes to patch artificially created low-degree nodes via corruptions, aiming at progressively reconstructing target GNN's predictions over a sequence of increasingly corrupted nodes. Through this scheme, GraphPatcher not only learns how to enhance low-degree nodes (when the neighborhoods are heavily corrupted) but also preserves the original superior performance of GNNs on high-degree nodes (when lightly corrupted). Additionally, GraphPatcher is model-agnostic and can also mitigate the degree bias for either self-supervised or supervised GNNs. Comprehensive experiments are conducted over seven benchmark datasets and GraphPatcher consistently enhances common GNNs' overall performance by up to 3.6% and low-degree performance by up to 6.5%, significantly outperforming state-of-the-art baselines. The source code is publicly available at https://github.com/jumxglhf/GraphPatcher.

==> table1_updated.tex <==
\begin{table}
\begin{center}
\caption{Updated Table 1 with heterophilic graphs.} 
\resizebox{1\columnwidth}{!}{
\begin{tabular}{l|ccccccccc}
\toprule
% \toprule
Method & \texttt{Cora} & \texttt{Citeseer} & \texttt{Pubmed} & \texttt{Wiki.CS} & \texttt{Am.Photo} & \texttt{Co.CS} & \texttt{Arxiv} & \texttt{Chameleon} & \texttt{Actor} \\
\midrule
\multicolumn{10}{c}{\textsc{Accuracy on Low-degree Nodes (Lower Percentile)}} \\
\cmidrule(r){1-10} 
\gcn      & 73.27$_{\pm{0.01}}$ & 64.86$_{\pm{0.92}}$ & 76.88$_{\pm{0.40}}$ & 72.98$_{\pm{0.50}}$ & 75.59$_{\pm{0.43}}$ & 84.59$_{\pm{0.45}}$ & 63.15$_{\pm{0.13}}$ & 54.05$_{\pm{0.18}}$ & 27.30$_{\pm{0.52}}$\\
\coldbrew & 73.82$_{\pm{0.98}}$ & \underline{65.60$_{\pm{0.08}}$} & \underline{77.72$_{\pm{0.63}}$} & 73.98$_{\pm{0.52}}$ & 76.18$_{\pm{0.80}}$ & \underline{85.56$_{\pm{0.69}}$} & 63.02$_{\pm{0.21}}$ & 53.41$_{\pm{0.22}}$ & \second{27.88}$_{\pm{0.13}}$ \\
\tailgnn  & 71.17$_{\pm{0.80}}$ & 57.66$_{\pm{0.83}}$ & 75.38$_{\pm{0.89}}$ & \best{74.36$_{\pm{0.18}}$} & \underline{77.22$_{\pm{0.94}}$} & 85.13$_{\pm{0.60}}$ & OOM & 53.48$_{\pm{0.04}}$ & 27.80$_{\pm{0.62}}$\\
\tuneup   & \underline{74.47$_{\pm{0.34}}$} & 65.17$_{\pm{0.22}}$ & 77.18$_{\pm{0.39}}$ & 72.60$_{\pm{0.75}}$ & 76.08$_{\pm{0.62}}$ & 84.68$_{\pm{0.50}}$ & \underline{63.34$_{\pm{0.32}}$} & 53.87$_{\pm{0.43}}$ & 27.94$_{\pm{0.14}}$\\
\eerm     & 73.40$_{\pm{0.06}}$ & 64.27$_{\pm{0.33}}$ & 76.30$_{\pm{0.20}}$ & 73.12$_{\pm{0.68}}$ & 75.15$_{\pm{0.59}}$ & 84.82$_{\pm{0.74}}$ & 63.20$_{\pm{0.11}}$ & \second{54.11}$_{\pm{0.32}}$ & 27.48$_{\pm{0.39}}$ \\
\gtrans   & 73.16$_{\pm{0.66}}$ & 64.95$_{\pm{0.83}}$ & 77.05$_{\pm{1.00}}$ & 72.15$_{\pm{0.50}}$ & 75.55$_{\pm{0.55}}$ & 84.74$_{\pm{0.06}}$ & 62.88$_{\pm{0.14}}$ & 54.29$_{\pm{0.14}}$ & 27.53$_{\pm{0.21}}$ \\
\dropedge & 73.57$_{\pm{0.97}}$ & 65.47$_{\pm{0.27}}$ & 75.68$_{\pm{0.82}}$ & 73.94$_{\pm{0.20}}$ & 76.49$_{\pm{0.03}}$ & 84.31$_{\pm{0.33}}$ & 61.33$_{\pm{0.33}}$ & 54.12$_{\pm{0.41}}$ & 27.39$_{\pm{0.24}}$ \\
\method   & \best{78.08$_{\pm{0.06}}$} & \best{67.27$_{\pm{0.20}}$} & \best{78.98$_{\pm{0.21}}$} & \underline{74.04$_{\pm{0.86}}$} & \best{77.84$_{\pm{0.36}}$} & \best{86.76$_{\pm{0.84}}$} & \best{64.01$_{\pm{0.12}}$} & \best{54.48}$_{\pm{0.71}}$ & \best{29.27}$_{\pm{0.57}}$\\
\cmidrule(r){1-10} 
\multicolumn{10}{c}{\textsc{Accuracy on High-degree Nodes (Upper Percentile)}} \\
\cmidrule(r){1-10} 
\gcn      & 86.83$_{\pm{0.17}}$ & \best{77.25$_{\pm{1.00}}$} & 80.84$_{\pm{0.76}}$ & 83.40$_{\pm{0.70}}$ & 84.07$_{\pm{0.71}}$ & \second{90.20$_{\pm{0.37}}$} & 80.46$_{\pm{0.18}}$ & 54.11$_{\pm{0.73}}$ & 27.41$_{\pm{0.29}}$ \\
\coldbrew & 84.80$_{\pm{0.04}}$ & 75.33$_{\pm{0.84}}$ & 78.66$_{\pm{0.38}}$ & 71.98$_{\pm{0.95}}$ & 77.07$_{\pm{0.14}}$ & 82.16$_{\pm{0.39}}$ & 70.57$_{\pm{0.36}}$ & 53.72$_{\pm{0.48}}$ & 26.67$_{\pm{0.29}}$ \\
\tailgnn  & 84.13$_{\pm{0.48}}$ & 74.85$_{\pm{0.30}}$ & 78.74$_{\pm{0.34}}$ & 78.91$_{\pm{0.97}}$ & 80.32$_{\pm{0.60}}$ & 86.75$_{\pm{0.90}}$ & OOM & \best{54.53}$_{\pm{0.12}}$ & 27.13$_{\pm{0.44}}$ \\
\tuneup   & \second{87.13$_{\pm{0.67}}$} & \second{76.95$_{\pm{0.63}}$} & \second{81.74$_{\pm{0.49}}$} & 83.11$_{\pm{0.53}}$ & 81.57$_{\pm{0.07}}$ & 90.65$_{\pm{0.86}}$ & 80.09$_{\pm{0.51}}$ & 54.25$_{\pm{0.59}}$ & 26.64$_{\pm{0.71}}$ \\
\eerm     & 85.89$_{\pm{0.09}}$ & 76.32$_{\pm{0.23}}$ & 79.98$_{\pm{0.06}}$ & 82.98$_{\pm{0.07}}$ & \second{84.32$_{\pm{0.96}}$} & 90.17$_{\pm{0.11}}$ & 80.37$_{\pm{0.12}}$ & \second{54.41}$_{\pm{0.71}}$ & \second{27.39}$_{\pm{0.14}}$ \\
\gtrans   & 86.32$_{\pm{0.34}}$ & 76.60$_{\pm{0.44}}$ & 80.56$_{\pm{0.92}}$ & \second{83.42$_{\pm{0.04}}$} & 83.95$_{\pm{0.99}}$ & 89.99$_{\pm{0.10}}$ & \best{80.77$_{\pm{0.26}}$} & 54.21$_{\pm{0.19}}$ & 27.29$_{\pm{0.12}}$ \\
\dropedge & 86.53$_{\pm{0.99}}$ & 76.35$_{\pm{0.17}}$ & 81.44$_{\pm{0.51}}$ & 83.37$_{\pm{0.43}}$ & \best{84.97$_{\pm{0.56}}$} & 89.28$_{\pm{0.08}}$ & \second{80.64$_{\pm{0.36}}$} & 54.17$_{\pm{0.11}}$ & 27.38$_{\pm{0.21}}$ \\
\method   & \best{88.02$_{\pm{0.11}}$} & 76.65$_{\pm{0.18}}$ & \best{83.83$_{\pm{0.79}}$} & \best{83.49$_{\pm{0.22}}$} & 84.17$_{\pm{0.97}}$ & \best{90.59$_{\pm{0.46}}$} & 80.61$_{\pm{0.25}}$ & 54.20$_{\pm{0.21}}$ & \best{27.43}$_{\pm{0.62}}$ \\
\cmidrule(r){1-10} 
\rowcolor{gray!12} \multicolumn{10}{c}{\textsc{Overall Performance}} \\
\cmidrule(r){1-10} 
\gcn      & 81.22$_{\pm{0.40}}$ & 70.51$_{\pm{0.46}}$ & 79.14$_{\pm{0.31}}$ & 77.30$_{\pm{0.41}}$ & 80.38$_{\pm{0.86}}$ & 88.16$_{\pm{0.66}}$ & 71.73$_{\pm{0.14}}$ & 52.83$_{\pm{0.35}}$ & 27.20$_{\pm{0.57}}$ \\
\coldbrew & 80.70$_{\pm{0.86}}$ & 70.10$_{\pm{0.55}}$ & 78.66$_{\pm{0.93}}$ & 73.82$_{\pm{0.69}}$ & 78.24$_{\pm{0.62}}$ & 85.80$_{\pm{0.79}}$ & 63.55$_{\pm{0.48}}$ & 52.12$_{\pm{0.53}}$ & 26.75$_{\pm{0.32}}$ \\
\tailgnn  & 79.44$_{\pm{0.64}}$ & 65.80$_{\pm{0.04}}$ & 76.14$_{\pm{0.25}}$ & 74.66$_{\pm{0.18}}$ & 80.68$_{\pm{0.58}}$ & 87.02$_{\pm{0.33}}$ & OOM  & 52.46$_{\pm{0.12}}$ & \second{27.62}$_{\pm{0.47}}$ \\
\tuneup   & \second{82.11$_{\pm{0.39}}$} & 70.92$_{\pm{0.02}}$ & \second{79.91$_{\pm{0.26}}$} & 76.93$_{\pm{0.81}}$ & 79.74$_{\pm{0.28}}$ & \second{88.46$_{\pm{0.97}}$} & 71.51$_{\pm{0.30}}$  & 52.89$_{\pm{0.41}}$ & 27.32$_{\pm{0.64}}$ \\
\eerm     & 81.47$_{\pm{0.19}}$ & 70.08$_{\pm{0.19}}$ & 78.65$_{\pm{0.43}}$ & 77.29$_{\pm{0.96}}$ & 79.79$_{\pm{0.61}}$ & 88.07$_{\pm{0.30}}$ & 71.70$_{\pm{0.18}}$ & \second{52.93}$_{\pm{0.24}}$ & 27.65$_{\pm{0.29}}$ \\
\gtrans   & 80.79$_{\pm{0.51}}$ & 69.51$_{\pm{0.93}}$ & 78.67$_{\pm{0.93}}$ & 76.39$_{\pm{0.27}}$ & 80.02$_{\pm{0.80}}$ & 88.06$_{\pm{0.96}}$ & 71.77$_{\pm{0.19}}$ & 52.67$_{\pm{0.35}}$ & 26.93$_{\pm{0.41}}$ \\
\dropedge & 81.10$_{\pm{0.31}}$ & \second{71.10$_{\pm{0.86}}$} & 78.90$_{\pm{0.68}}$ & \second{77.49$_{\pm{0.78}}$} & \second{81.11$_{\pm{0.72}}$} & 87.56$_{\pm{0.64}}$ & \second{71.82$_{\pm{0.33}}$} & 52.89$_{\pm{0.22}}$ & 27.28$_{\pm{0.32}}$ \\
\method   & \best{84.17$_{\pm{0.54}}$} & \best{71.65$_{\pm{0.05}}$} & \best{81.13$_{\pm{0.68}}$} & \best{78.12$_{\pm{0.57}}$} & \best{81.23$_{\pm{0.32}}$} & \best{89.44$_{\pm{0.79}}$} & \best{72.31$_{\pm{0.22}}$}  & \best{53.21}$_{\pm{0.39}}$ & \best{28.34}$_{\pm{0.24}}$ \\
% \bottomrule
\bottomrule
\end{tabular}}
\vspace{-0.05in}
\label{tab:table1_update}
\end{center}
\end{table}
